ReSpAct: Harmonizing Reasoning, Speaking, and Acting Towards Building Large Language Model-Based Conversational AI Agents

Large language model (LLM)-based agents are increasingly employed to interact with external environments (e.g., games, APIs, world models) to solve user-provided tasks. However, current frameworks often lack the ability to collaborate effectively with users in fully conversational settings. Conversations are essential for aligning on task details, achieving user-defined goals, and satisfying preferences. While existing agents address ambiguity through clarification questions, they underutilize the broader potential of an LLM's conversational capabilities. In this work, we introduce ReSpAct, an LLM-based agent designed to seamlessly integrate reasoning, decision-making, and dynamic dialogue for task-solving. Expanding on reasoning-first approaches like ReAct, ReSpAct employs active, free-flowing dialogues to interpret instructions, clarify goals, provide status updates, resolve subtask failures, and refine plans based on user inputs without any explicit dialogue schema. By alternating between task-solving actions and interactive conversations, ReSpAct demonstrates improved performance across diverse environments. We evaluate ReSpAct in user-interactive settings, including task-oriented dialogue systems (MultiWOZ) and decision-making tasks (ALFWorld, WebShop). ReSpAct outperforms ReAct with absolute success rate improvements of 6% and 4% in ALFWorld and WebShop, respectively, and achieves a 5.5% gain in Inform and a 3% gain in Success scores in MultiWOZ. These results highlight the value of integrating dynamic user-agent collaboration for more effective task resolution.

==> acl_2025_sections/table/human_eval.tex <==
% \begin{table}[!h]
% \scriptsize
% \begin{minipage}{1.0\linewidth}
%     \centering
% \begin{tabular}{l|clll}
% \toprule
%     & Type & Definition & \react & \respact \\
% \midrule
% \multirow{2}{*}{Success} & True positive & Correct reasoning trace and facts & \% & \% \\ & False positive & Hallucinated reasoning trace or facts & \% & \%\\
%     \hline
%     \multirow{4}{*}{Failure} & Reasoning error & Wrong reasoning trace (including failing to recover from repetitive steps) & \% & \% \\ & Search result error & Search return empty or does not contain useful information & \% & - \\ & Hallucination & Hallucinated reasoning trace or facts & \% & \% \\ & Label ambiguity & Right prediction but did not match the label precisely & \% & \%\\
% \bottomrule
% \end{tabular}
% \caption{
% Types of success and failure modes of \model{} and \reason{} on AlfWorld, as well as their percentages in randomly selected examples studied by human.
% }
% \label{table:human_study_categories}
% \end{minipage}%
% \vspace{-10pt}
% \end{table}

% \begin{table}[t]
% \centering
% \scriptsize
% \begin{tabular}{l|l|l|c|c}
% \hline
%  & Type & Definition & ReAct & ReSpAct \\
% \hline
% \multirow{2}{*}{Success} & True positive & Correct reasoning trace and facts & \% & \% \\
%  & False positive & Hallucinated reasoning trace or facts & \% & \% \\
% \hline
% \multirow{4}{*}{Failure} & Reasoning error & Wrong reasoning trace (including failing to recover from repetitive steps) & \% & \% \\
%  & Search result error & Search return empty or does not contain useful information & \% & - \\
%  & Hallucination & Hallucinated reasoning trace or facts & \% & \% \\
%  & Label ambiguity & Right prediction but did not match the label precisely & \% & \% \\
% \hline
% \end{tabular}
% \caption{Types of success and failure modes of ReAct and ReSpAct on AlfWorld, as well as their percentages in randomly selected examples studied by human.}
% \label{table:human_study_categories}
% \end{table}

\begin{table*}
  \centering
  \small
  \begin{tabular}{l|l|l|c|c}
    \hline
    \textbf{}                & \textbf{Type}            & \textbf{Definition}        & \textbf{ReAct} & \textbf{ReSpAct} \\
    \hline
    \multirow{2}{*}{Success} & True positive            & Correct reasoning trace and facts               & \%               & \% \\
                             & False positive           & Hallucinated reasoning trace or facts           & \%               & \% \\
    \hline
    \multirow{4}{*}{Failure} & Reasoning error          & Wrong reasoning trace (including failing to recover from repetitive steps) & \% & \% \\
                             & Hallucination            & Hallucinated reasoning trace or facts           & \%               & \% \\
                             & Label ambiguity          & Right prediction but did not match the label precisely & \%        & \% \\
    \hline
  \end{tabular}
  \caption{\label{table:human_study_categories}
    Types of success and failure modes of ReAct \& ReSpAct on AlfWorld, as well as their percentages in randomly selected examples studied by human.
  }
\end{table*}

